Probing dark matter substructure in the gravitational lens HE0435-1223 with the WFC3 grism

Strong gravitational lensing provides a powerful test of Cold Dark Matter (CDM) as it enables the detection and mass measurement of low mass haloes even if they do not contain baryons. Compact lensed sources such as Active Galactic Nuclei (AGN) are particularly sensitive to perturbing subhalos, but their use as a test of CDM has been limited by the small number of systems which have significant radio emission which is extended enough avoid significant lensing by stars in the plane of the lens galaxy, and red enough to be minimally affected by differential dust extinction. Narrow-line emission is a promising alternative as it is also extended and, unlike radio, detectable in virtually all optically selected AGN lenses. We present first results from a WFC3 grism narrow-line survey of lensed quasars, for the quadruply lensed AGN HE0435-1223. Using a forward modelling pipeline which enables us to robustly account for spatial blending, we measure the [OIII] 5007 \AA~ flux ratios of the four images. We find that the [OIII] fluxes and positions are well fit by a simple smooth mass model for the main lens. Our data rule out a $M_{600}>10^{8} (10^{7.2}) M_\odot$ NFW perturber projected within $\sim$1\farcs0 (0\farcs1) arcseconds of each of the lensed images, where $M_{600}$ is the perturber mass within its central 600 pc. The non-detection is broadly consistent with the expectations of $\Lambda$CDM for a single system. The sensitivity achieved demonstrates that powerful limits on the nature of dark matter can be obtained with the analysis of $\sim20$ narrow-line lenses.

==> refereeResponse.tex <==
Assistant Editor's Comments:

Please ensure that all references to arxiv papers also include the preprint number, e.g. arXiv:1506.08817.



Reviewer's Comments:

This is an interesting paper, presenting a novel data analysis technique which
should enable the authors and the wider community to improve our current
constraints on the mass function of dark matter subhalos using the HST/WFC3
grism. I have no major concerns with the data analysis or modeling approach,
and recommend that this work be published after some minor concerns are
addressed.

Mostly minor issues:

The authors should provide the lens model parameters (e.g., Einstein
radius, ellipticity, etc.) and uncertainties, and compare these to those
derived from other works, in particular those which model broad-line or
continuum bands. Does the microlensing of image A significantly alter
the model parameters?

> The lens model parameters with one sigma uncertainties are listed in Table 1. We have added a few sentences comparing these lens model parameters with other results from the literature to at the end of the second paragraph of Section 5.1. Unfortunately the study that was affected by microlensing did not publish their lens model parameters and thus we cannot compare. We've added a sentence stating this at the beginning of the third paragraph of Section 5.1 


The authors imply several times that their method is largely immune to 
differential extinction due to dust within the lens galaxy (e.g., abstract,
S7), similar to the radio continuum emission. However, the reason for this
is never explained very clearly. The authors may wish to summarize that
reasoning (Moustakas & Metcalf 2003), and also point out that there has
been no evidence of significant dust in this particular lens (Wisotzki et al. 
2003).

> We have added a paragraph to the end of Section 3.2 discussing this assumption in more detail.



Could the authors comment on whether the nearby object G2 can be
effectively modeled as contributing to external shear for their purposes, 
even though they are not modeling the time delays? Sluse et al. (2017), for 
example, find that G2 significantly perturbs the lens potential even though
it is behind the main lens, and should be explicitly included in lens models
of this system. 

> We have added some clarifying remarks in the text. Sluse et al. (2016) found that G1 (formerly known as G2 in our paper, aka the nearby galaxy) might have an effect on percent level inferences on H0. However for our purposes, the fact that the image positions are well fit by a simple one lens system indicates that this level of model complexity is sufficient. Reassuringly, we find similar lens Einstein radius and external shear magnitudes to those found by Sluse et al. 2012, who modelled the HE0435 positions with only a single lens galaxy. We have added this reference to the text, and emphasized that we allow the macromodel to freely vary.  

Even more minor comments:

- The H0LICOW papers all refer to the galaxy here called G2 as G1. The
authors may wish to match this nomenclature for the sake of the 
collective sanity of the literature.

>Fixed!


- Abstract, final sentence - can the authors give the number of systems to be
included in "the entire sample"?

>We have added ~20

- Page 2, left column, sentence beginning "Strong gravitational lensing..." -
This sentence may be overstated - as the authors note, the perturbations from
subhalos of a given mass are also strongly dependent on the shape of the mass 
profile, which of course is even more difficult than constraining the mass
profile for the main lens itself.

> We have modified this sentence to clarify that we meant that the subhalo mass function measurement does not require stars or gas to detect the subhalos (rather than claiming that it is independent of baryons).


- Page 2, left column, end of paragraph above - On the other end of the size
scale, the authors may wish to note that large background sources (~several 
kpc) also present a challenge for lens modeling because the intrinsic source 
structure is mostly unknown, but probably complex. The narrow line technique
hits a bit of a sweet spot between source emission that is sufficiently
extended but not yet too complex.
>We have added a sentence stating this.

- Page 2, left column, last paragraph - Please note the typical size scale
of the radio continuum emission.
>added

- Page 3, beginning of S3 - "quasar images and galaxies from in a model"
>fixed
- S3.1 - First sentence should be two sentences, split at "direct image. 
Thus... "
>fixed

- S3.1 - "We have tested several different..." - I assume that the image
positions also are not sensitive to the galaxy model used; this should be 
noted for completeness.
>We have added a sentence explicitly stating this



- S3.2 - "We model the continuum emission over..." - Is the reason a linear
continuum was used instead of a power-law simply that the fractional 
wavelength coverage is small?
>Yes, we've added an explicit statement of this in the text.


- S3.2 - "The ratio of the [OIII] doublet 4959 and 5007..." - some justification
for the 1/3 ratio should be given.
>Clarified

- S7, paragraph beginning "We further assume..." - Could the authors clarify
whether the expectation of ~15 subhalos of M > 10^7 Msun assumes the full
~5kpc exclusion radius, or the (much smaller) area of sensitivity to the
lower mass subhalos? As currently phrased, this paragraph makes it sound 
quite surprising that no subhalos of 10^7 Msun were detected (because ~15
were expected, even given the uncertainties in that number).




%>We are very grateful that the referee caught this. Indeed, we had mistakenly not scaled the 10^7 Msun value to the correct sensitivity area. We have revised this number to only integrate over satellites in the sensitivity region.

- Figure 1 - Can the x axis of the grism images be labeled with "\lambda -->",
just to show the direction of increasing wavelength? Otherwise this figure is
very well done.
>Fixed

- Figure 2 - Can the Hbeta and [OIII] lines be labeled or pointed out with 
arrows in at least one of the sub-panels?
>Added

- Figure 3 - Can the Hbeta and [OIII] text labels be moved below the data
points? Also, in the caption - "Measurements in the same filter have years are
slightly offset...".

>Hbeta OIII labels moved, and caption fixed

Figure 8 - I may be mistaken, but it appears the left panels show the narrow
line emission alone, while the right panels also include the broad-line emission
(otherwise I don't see a correspondence between the sets of panels). This should
be noted, if so.

>We've clarified this in the caption.



